RadLing: Towards Efficient Radiology Report Understanding

Most natural language tasks in the radiology domain use language models pre-trained on biomedical corpus. There are few pretrained language models trained specifically for radiology, and fewer still that have been trained in a low data setting and gone on to produce comparable results in fine-tuning tasks. We present RadLing, a continuously pretrained language model using Electra-small (Clark et al., 2020) architecture, trained using over 500K radiology reports, that can compete with state-of-the-art results for fine tuning tasks in radiology domain. Our main contribution in this paper is knowledge-aware masking which is a taxonomic knowledge-assisted pretraining task that dynamically masks tokens to inject knowledge during pretraining. In addition, we also introduce an knowledge base-aided vocabulary extension to adapt the general tokenization vocabulary to radiology domain.

==> rough.tex <==
To the best of our knowledge, ours is the first work that utilizes domain knowledge in the form of....

\begin{itemize}
    \item What are radiology reports? Why are they important to doctors?
    \item How does BERT architectures help in radiology nlp --> Say cool things about them and then go to your example. Start with this sentence, However, some challenges remain when adapting these models as is, to radiology reports. Let us look at an example from , (Bring your example here). Here there is a problem, 

    Approaches like RadBERT try to solve this problem by using radiology reports as their training corpus. However, problems still remain because radiology reports are often dense with information and terse in length. This ends up causing problems during (Random masking issues) that hook here,

    To address these issues we introduce our model RadLing, which utilizes a domain specific training objective.... bll b, 

    our contributions can be summarized as : 

    \begin{enumerate}
        \item 1, 2 and 3
    \end{enumerate}
        
    Background : In this paper we introduce - a, b and c. So the related work spans - continuous pretraining, better contextualization architectures, knowledge injection into LLMs, 
    \item What are the challenges that remain? (Bring the example)
    \item What is our solution to solve this challenge?
    \item Why is it non trivial?
    \item in summary our contributions in this paper are:
\end{itemize}

High-performing PLMs that are publicly available are large. PubmedBERT has 109 million parameters and the best performing RadBERT variant has 125 million parameters. In an industrial deployment setting, larger models have latency issues.

\begin{itemize}
    \item Radiology report 
\end{itemize}

Radiology NLU can potentially aid in summarising patient imaging history, cost-effective medical image annotation, quick information extraction and summarisation for healthcare professionals. This helps in building robust clinical decision support systems. These applications can also provide downstream assistance to biomedical research in the form of discovery of new phenotypes and links between biomedical concepts, capturing knowledge and intuition of experienced radiologists, and tracking of patient response to therapy through findings in medical images.
The models currently used in radiology domain sometimes have problems understanding context of entities. These models are pretrained using BERT-like architectures and use Masked Language modeling (MLM) as their objectives. However, in radiology reports, every sentence has multiple concepts, and the relation between these concepts are not always explicit. Random masking in Masked language modeling (MLM) is already known to have context understanding issues\citep{song2020mpnet}. Such issues mostly stem from information loss due to masking key context clues in the text and non contiguous masking problems. We have noticed finetuned models of RadBERT and PubmedBERT failing to identify relations in ambiguous sentences. RadGraph benchmarking \citep{jain2021radgraph} has reported lower F1 scores for relation labels like `Suggestive\_Of' (MIMIC-CXR: 0.685, CheXpert: 0.585). We surmise that these problems can be avoided with the help of domain knowledge. In radiology domain, an excellent source of domain knowledge is the taxonomical knowledge base RadLex\citep{langlotz2006radlex}, which curates radiology lexicons. Figure \ref{fig:ex} shows an example sentence which is ambiguous for a non-clinical person, and difficult for current state of the art models. However, a look at RadLex for the entity `Pneumonia' reveals its \textit{Anatomical\_site} property to be `Lungs'.

Other challenges faced by researchers in radiology-related natural language processing tasks include and are not limited to availability of large volumes of training data, formulation of domain-specific training objectives and method of domain knowledge integration. Use of large datasets like MIMIC-IV\citep{johnson2020mimic} might not be feasible for industry research due to license restrictions.  The purpose of RadLex is standardisation of radiology terms, and hence the efforts to populate it are less oriented towards knowledge graph completion. In addition, the aforementioned radiology language models are large: PubmedBERT has 109 million parameters and the best performing RadBERT variant has 125 million parameters. In an industrial deployment setting, larger models have latency issues. Reduction in parameters by quantisation or distillation also reduces efficiency which is less than ideal.

\subsection{Datasets}
%\subsubsection{Pretraining}
  
\subsubsection{Named Entity Recognition}
There are 12,388 and 2191 entities in the training and validation dataset of RadGraph dataset \citep{jain2021radgraph} respectively. In the test set, there are 1293 and 1473 entities in MIMIC-CXR and CheXpert respectively. Overall, we have an imbalanced dataset with less than 5\% uncertain observations. The evaluation criteria is class-level and aggregate macro F1 and micro F1. Radiologist benchmark macro F1s for this task are 0.981 and 0.894 for MIMIC-CXR and CheXpert respectively.

\subsubsection{Relationship Extraction}
We have used RadGraph dataset for this task. There are 9251 relations in the training dataset, 1638 in the validation dataset, 902 in MIMIC-CXR test dataset and 1107 in CheXpert dataset. This dataset is imbalanced with < 6\% of relations being `Suggestive of'. The evaluation metrics for this dataset are macro F1 and micro F1, both on an aggregate level and for each relationship class. Radiologist benchmark macro F1s for this task are 0.91 and 0.704 for MIMIC-CXR and CheXpert respectively.

\subsubsection{Abnormal Classification}
This downstream task is a binary classification problem and involves identification of reports that are normal versus the ones that indicate some abnormality in the image. The dataset\citep{demner2016preparing} contains 3996 de-identified reports, manually and independently annotated by two coders trained in medical informatics. There are 2564 abnormal reports and the rest are normal. The evaluation metrics for this dataset are macro- and micro-F1 on test dataset.

\subsubsection{Radiology Question Answering}
 There are 6148 questions in the RadQA dataset \citep{soni2022radqa}, among which 1745 are unanswerable, and the rest of the answers have median and average lengths of 7 and 16.2 respectively. The evaluation of this dataset uses standard Machine Reading Comprehension (MRC) \citep{gardner2019question} metrics, i.e., stricter metric Exact match (EM)  and F1 where word level match is calculated between reference and predicted answers. 

 RadLing increases contextual understanding of radiology reports with the help of domain-specific KG and pretraining objectives. 
 \textbf{Radiology report understanding using MLMs.} \cite{yan2022radbert} has used masked language modeling with several pretrained PLMs to train on radiology reports. RadBERT has experimented on training with 2.16 million and 4.4 million training repotrs with pretrained large language models like BERT, RoBERTa and Clinical BERT using Masked Language Modeling pretraining objective. It has been fine tuned on three tasks: abnormal sentence classification, report coding and classification. We have further tested these models for NER, RE, abnormal report classification and QA, and they have generated best results compared to other models. In contrast, we have trained with knowledge graph pretraining objectives on much smaller dataset with 545k reports, and achieved comparable results for NER, RE and Abnormals classification. 
 \textbf{Other biomedical pretraining objectives.} EntityBERT \cite{lin2021entitybert} used entity masking pretraining objective to infuse domain knowledge, in which 40\% of the entities and 12\% of random words are chosen respectively within each sequence block for corruption. They have used continuously pretrained PubMedBERT with MIMIC-III dataset \citep{johnson2016mimic}. This pretraining objective can mask context in radiology reports, and hence we improved on this by using RadLex. Section segmentation is another radiology-specific pretraining objective proposed in  BiRadsBERT \cite{kuling2021bi} which we have adapted to our work RadLing-SS. The sections used in BiRadBERT are Title, Patient History or Clinical Indication, Prior Imaging reference, Technique/Procedure Notes, Findings, Impression/Opinion, and Assessment Category. We only used Findings, Impression, Clinical history, Prior Imaging reference (comparison) and Miscellaneous as the sections in RadLing-SS. This is in keeping with the structure of our dataset.
\textbf{Biomedical Knowledge Graph infusion.} KeBioLM \citep{yuan-etal-2021-improving} applies text-only encoding layer to learn entity representation and applies a text-entity fusion encoding to aggregate entity representation. They train using three pretraining objectives: masked language modeling, which they extended to mask the entire entity, entity detection and entity linking to UMLS\citep{bodenreider2004unified}. They have surpassed state-of-the-art in biomedical NER and RE tasks. BioKGLM\cite{fei2021enriching} introduces a separate post-training procedure between pretraining and finetuning where they experimented several strategies using knowlede embedding algorithms to inject domain knowledge. They have compiled a large biomedical knowledge graph from various sources. RadLing uses radiology domain-specific knowledge graph RadLex and uses pretraining objectives like intelligent entity masking to enable better context understanding.

The vocabulary of the pretrained model is re- 122
tained in continuous pretraining, e.g., biomed- 123
ical BERT (BioBERT). One drawback of this 124
approach is that due to subword tokeniza- 125
tion used in the language models, some do- 126
main specific words get fragmented into non- 127
meaningful tokens. For example, BERT frag- 128
ments biomedical terms like ‘Thalamus’ into 129
‘Tha’, ‘##lam’, ‘##us’, thereby losing the 130
domain-specific meaning. 131
(b) Retraining a tokenizer from scratch using the 132
vocabulary from the in-domain documents, 133
e.g., SciBERT (Beltagy et al., 2019) and Pub- 134
medBERT. We have a comparatively smaller 135
set of documents in our corpus, and we are 136
continuously pretraining from existing model. 137
So this is not feasible for us. 138
(c) Extending the existing vocabulary to fit 139
domain-specific words, like tokenization in 140
exBERT(Tai et al., 2020) or AVocaDo (Hong 141
et al., 2021). We have used a modification of 142
AvoCado in our paper. 143
Our tokenization methods consists of the follow- 144
ing steps: 145
1. We perform Wordpiece tokenization on our 146
corpus to form the set of new tokens Tcorpus. 147
2. The vocabulary of BERT contains set of to- 148
kens TBERT . We find the tokens that belong 149
2

Discussion 
Despite using a smaller radiology report dataset for pretraining than the PLMs in other state-of-the-art systems, RadLing models are nonetheless able to match the performance of these systems on a number of fine-tuning tasks.
%RadLing has been trained on smaller radiology dataset compared to the other state-of-the-art systems, but the model has produced results on several finetuning tasks that are comparable to larger models trained on larger datasets. 
RadLing outperforms the state-of-the-art models for NER, RE and has the same performance as RadBERT in Abnormal classification. Additionally, in terms of size, RadLing has 13.7 million trainable parameters while the models being compared in this work, PubMedBERT and RadBERT, have 110 million and 125 million trainable parameters, respectively. We have tested the model on proprietary NER datasets, and the model has yielded 0.92-0.93 macro F1 on less represented anatomies like neck, while for the highly represented anatomies, F1 in the same dataset is as high as 0.98.

%Additionally, in terms of size, the number of trainable parameters in RadLing is 13.7M, while PubMedBERT and RadBERT models compared in this paper are 110M and 125M, respectively. 
The choice of Electra small is influenced by its unique architecture that has been shown to yield good results with less data. Transformer models generally produce better results with more data, thus we would like to train our architectures on larger datasets in future. In addition, we would also like a good balance of radiology imaging modalities and anatomies represented in the dataset. Furthermore, we would like to have reports that are more representative of the genders, races, and nations from which these datasets are sourced. 

We would like to explore more on knowledge graph infusion in our data. RadLex contains textual descriptions of the entities, and has many other properties that can be utilized for language model training. In addition, there are several other biomedical knowledge graphs that RadLex is directly connected to, like Snomed and UMLS. We can exploit a combination of knowledge graphs to enhance the information encoded in RadLing. We would also like to experiment with causal language modeling based architectures for pretraining in radiology domain. 

Conclusion
In this work we have explored a cost-effective method to train a high performing radiology PLM, RadLing with a small dataset. We developed a knowledge-aware masking strategy to use RadLex to infuse context into radiology PLMs to train RadLing-KG. This led us to the following observations. First, Electra architecture, without any special pretraining objectives, is able to produce good results with most of the downstream tasks. In a task like relationship extraction, it even outperforms Radgraph radiologist benchmarks. Second, RadLing-KG is the best performing RadLing variant, and outperforms the downstream task benchmarks in all the tasks except QA. Third, Domain specific vocabulary is helpful in better performance of models, In addition, in tasks that use cross attention like vision-language tasks or explainable AI, having unfragmented radiology tokens is helpful. For example, BERT fragments biomedical terms like ‘Thalamus’ into 129
‘Tha’, ‘##lam’, ‘##us’, thereby losing the domain-specific meaning, whereas in our work, due to domain specific tokenization, the word 'Thalamus' is retained. Fourth, Infusion of RadLex information  counteracts Electra limitations in QA dataset. Finally, we have tested the model on proprietary NER datasets and RadLing-KG has yielded 0.92-0.93 macro F1 on less represented anatomies like neck, while for the highly represented anatomies, F1 is as high as 0.98. This actually shows the potential of using RadLex in radiology pretraining. Thus, in a real world setting with high imbalances in datasets, RadLing-KG is more robust.

In future we would like to explore more ways to infuse knowledge by 
\begin{inparaenum}
\item Using text description of context like \cite{yuan-etal-2021-improving},
\item Retrieving more context from biomedical knowledge graphs like SNOMED \footnote{https://www.nlm.nih.gov/healthit/snomedct/index.html} and UMLS, and
\item more robust knowledge embedding methods.
\end{inparaenum}
We would also like to experiment with larger datasets and models, and work with more downstream radiology applications.

\begin{enumerate}
    \item We perform Wordpiece tokenization on our corpus to form the set of new tokens $\mathbb{T}_{corpus}$. 
    \item The vocabulary of BERT contains set of tokens $\mathbb{T}_{BERT}$. We find the tokens that belong to $\mathbb{T}_{corpus} - \mathbb{T}_{BERT}$ and call them  $\mathbb{T}_{candidate}$. We query RadLex to check whether the tokens in $\mathbb{T}_{candidate}$ represent any concept in RadLex. In case the word is present in RadLex, we append the token to the new set of tokens $\mathbb{T}_{new}$.
    \item %We also introduce a set of special tokens $\mathbb{T}_s$ to the extended vocabulary. 
    Since the reports are anonymized, the names, dates and several other patient identifiers are replaced by fixed special tokens, such as `[date]', `[person]', `[location]', `[time]' and `[removed]'. We also include these sets of tokens $\mathbb{T}_s$ into our vocabulary.
    \item Our new vocabulary $\mathbb{T}_{RadLing} = \mathbb{T}_{BERT} + \mathbb{T}_{new} + \mathbb{T}_s$
\end{enumerate}


